SAGS: Structure-Aware 3D Gaussian Splatting

Following the advent of NeRFs, 3D Gaussian Splatting (3D-GS) has paved the way to real-time neural rendering overcoming the computational burden of volumetric methods. Following the pioneering work of 3D-GS, several methods have attempted to achieve compressible and high-fidelity performance alternatives. However, by employing a geometry-agnostic optimization scheme, these methods neglect the inherent 3D structure of the scene, thereby restricting the expressivity and the quality of the representation, resulting in various floating points and artifacts. In this work, we propose a structure-aware Gaussian Splatting method (SAGS) that implicitly encodes the geometry of the scene, which reflects to state-of-the-art rendering performance and reduced storage requirements on benchmark novel-view synthesis datasets. SAGS is founded on a local-global graph representation that facilitates the learning of complex scenes and enforces meaningful point displacements that preserve the scene's geometry. Additionally, we introduce a lightweight version of SAGS, using a simple yet effective mid-point interpolation scheme, which showcases a compact representation of the scene with up to 24$\times$ size reduction without the reliance on any compression strategies. Extensive experiments across multiple benchmark datasets demonstrate the superiority of SAGS compared to state-of-the-art 3D-GS methods under both rendering quality and model size. Besides, we demonstrate that our structure-aware method can effectively mitigate floating artifacts and irregular distortions of previous methods while obtaining precise depth maps. Project page https://eververas.github.io/SAGS/.

==> Tables/tab_TanksandTemples.tex <==
\begin{table}[ht]
\centering
\caption{\textbf{Per-scene rendering quality evaluation for Tanks\&Temples~\cite{Knapitsch2017} and Deep Blending~\cite{hedman2018deep} datasets.}}
\label{tab:tandt_dp}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccccccccccccccc}
\toprule
Scene & \multicolumn{3}{c}{Truck} & \multicolumn{3}{c}{Train} & \multicolumn{3}{c}{Dr Johnson} & \multicolumn{3}{c}{Playroom} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
Method & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS \\
\midrule

{3D-GS~\cite{kerbl3Dgaussians}} & 
25.19 & 0.879 & 0.148 &
21.10 & 0.802 & \cellcolor{tabthird}0.218 &
28.77 & 0.899 & \cellcolor{tabthird}0.244 &
\cellcolor{tabthird}30.04 & \cellcolor{tabsecond}0.906 & \cellcolor{tabfirst}{0.241} \\

{Mip-NeRF360~\cite{barron2022mipnerf360}} &
24.91 & 0.857 & 0.159 &
19.52 & 0.660 & 0.354 &
\cellcolor{tabthird}29.14 & \cellcolor{tabthird}0.901 & \cellcolor{tabsecond}0.237 &
29.66 & 0.900 & \cellcolor{tabthird}0.252 \\

{iNPG~\cite{muller2022instant}} & 23.26 & 0.779 & 0.274 & 20.17 & 0.666 & 0.386 & 27.75 & 0.839 & 0.381 & 19.48 & 0.754 & 0.465 \\

{Plenoxels~\cite{yu2022plenoxels}} & 23.22 & 0.774 & 0.335 & 18.93 & 0.663 & 0.422 & 23.14 & 0.787 & 0.521 & 22.98 & 0.802 & 0.499 \\

{Scaffold-GS~\cite{lu2023scaffold}} & 
    \cellcolor{tabthird}25.77 & \cellcolor{tabsecond}0.883 & \cellcolor{tabthird}0.147 & 
    \cellcolor{tabthird}22.15 & \cellcolor{tabsecond}0.822 & \cellcolor{tabsecond}0.206 & 
    \cellcolor{tabsecond}29.80 & \cellcolor{tabsecond}0.907 & 0.250 & 
    \cellcolor{tabsecond}{30.62} & \cellcolor{tabthird}0.904 & 0.258 \\
\midrule
{SAGS-Lite} & 
    \cellcolor{tabsecond}{25.95} & \cellcolor{tabthird}{0.881} & \cellcolor{tabsecond}{0.143} & 
    \cellcolor{tabsecond}{22.36} & \cellcolor{tabthird}{0.810} & {0.220} & 
    {28.61} & {0.890} & {0.285} 
    & {29.53} & {0.888} & {0.300} \\

{SAGS} & 
    \cellcolor{tabfirst}{26.31} & \cellcolor{tabfirst}{0.894} & \cellcolor{tabfirst}{0.134} & 
    \cellcolor{tabfirst}{23.44} & \cellcolor{tabfirst}{0.837} & \cellcolor{tabfirst}{0.198} & 
    \cellcolor{tabfirst}{29.99} & \cellcolor{tabfirst}{0.912} & \cellcolor{tabfirst}{0.234} & 
    \cellcolor{tabfirst}{30.96} & \cellcolor{tabfirst}{0.913} & \cellcolor{tabsecond}0.248 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> Tables/tab_bungeenerf.tex <==
\begin{table}[ht]
\centering
\caption{\textbf{Scores for Bungeenerf~\cite{xiangli2022bungeenerf} scenes.}}
\label{tab:bungeenerf}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
Scene & \multicolumn{3}{c}{Amsterdam} & \multicolumn{3}{c}{Bilbao} & \multicolumn{3}{c}{Pompidou} & \multicolumn{3}{c}{Quebec} & \multicolumn{3}{c}{Rome} & \multicolumn{3}{c}{Hollywood} \\
\midrule
Method & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS \\
\midrule

\textbf{3D-GS~\cite{kerbl3Dgaussians}} & 
25.74 & - & - & 
26.35 & - & - &  
21.20 & - & - & 
28.79 & - & - &  
23.54 & - & - & 
23.25 & - & -  \\

\textbf{Scaffold-GS} &
27.10 & - & - & 
27.66 & - & - & 
25.34 & - & - & 
30.51 & - & - & 
26.50 & - & - & 
24.97 & - & -  \\
\midrule

\textbf{SAGS-Lite} &
% amsterdam
 - & - & - &  
% bilbao
 27.12 & - & - &  
% pompidou
 - & - & - &  
% quebec
 - & - & - &  
% rome
 - & - & - &  
% hollywood
 - & - & -  \\ 

\textbf{SAGS} 
% amsterdam
& \textbf{27.48} & 0.908 & 0.143 
% bilbao
& \textbf{27.91} & 0.893 & 0.162 
% pompidou
& \textbf{25.54} & 0.858 & 0.208 
% quebec
& \textbf{30.53} & 0.942 & 0.137
% rome
& \textbf{26.46} & 0.81 & 0.181
% hollywood
& \textbf{24.76} & 0.791 & 0.288 \\
\bottomrule
\end{tabular}}
\end{table}

==> Tables/tab_bungeenerf_combined.tex <==
\begin{table}[ht]
\centering
\caption{\textbf{PSNR (dB) and Storage size (MB) for BungeeNeRF~\cite{xiangli2022bungeenerf} scenes.}}
\label{tab:bungeenerf}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\toprule
Scene & \multicolumn{2}{c}{Amsterdam} & \multicolumn{2}{c}{Bilbao} & \multicolumn{2}{c}{Pompidou} & \multicolumn{2}{c}{Quebec} & \multicolumn{2}{c}{Rome} & \multicolumn{2}{c}{Hollywood} \\
\midrule
Method & PSNR & Mem & PSNR & Mem & PSNR & Mem & PSNR & Mem  & PSNR & Mem  & PSNR & Mem  \\
\midrule

3D-GS~\cite{kerbl3Dgaussians} & 
25.74 & 1453 & 
26.35 & 1337 & 
21.20 & 2129 &
28.79 & 1438 & 
23.54 & 1626 & 
23.25 & 1642   \\

Scaffold-GS &
\cellcolor{tabsecond}27.10 & 243 &
\cellcolor{tabsecond}27.66 & 197 & 
\cellcolor{tabsecond}25.34 & 230 &
\cellcolor{tabsecond}30.51 & 166 &
\cellcolor{tabsecond}26.50 & 200 &  
\cellcolor{tabsecond}24.97 & 182   \\
\midrule

SAGS-Lite &
% amsterdam
 25.89 & \cellcolor{tabfirst}68 &  
% bilbao
 27.12 & \cellcolor{tabfirst}55 & 
% pompidou
 24.73 & \cellcolor{tabfirst}58 & 
% quebec
28.76 & \cellcolor{tabfirst}55 & 
% rome
 25.36 & \cellcolor{tabfirst}64 &
% hollywood
24.21 & \cellcolor{tabfirst}58   \\ 

SAGS
% amsterdam
& \cellcolor{tabfirst}{27.48} & \cellcolor{tabsecond}228 
% bilbao
& \cellcolor{tabfirst}{27.91} & \cellcolor{tabsecond}150
% pompidou
& \cellcolor{tabfirst}{25.54} & \cellcolor{tabsecond}177
% quebec
& \cellcolor{tabfirst}{30.72} & \cellcolor{tabsecond}113
% rome
& \cellcolor{tabfirst}{26.57} & \cellcolor{tabsecond}153
% hollywood
& \cellcolor{tabfirst}{25.21} & \cellcolor{tabsecond}132  \\
\bottomrule
\end{tabular}}
\end{table}

==> Tables/tab_bungeenerf_sizes.tex <==
\begin{table}[ht]
\centering
\caption{\textbf{Scores for Bungeenerf~\cite{xiangli2022bungeenerf} scenes.}}
\label{tab:bungeenerf_sizes}
\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{l|cccccc}
\toprule
Scene & Amsterdam & Bilbao & Pompidou & Quebec & Rome & Hollywood \\
\midrule

\textbf{3D-GS~\cite{kerbl3Dgaussians}} & 
1453 & 1337 & 2129 & 1438 & 1626 & 1642 \\

\textbf{Scaffold-GS} &
243 & 197 & 230 &  166 & 200 & 182 \\
\midrule

\textbf{SAGS-Lite} &
 - & 55 & - & - & - & -   \\ 

\textbf{SAGS} 
& 228.1 (2.3M) & 150 (1.52M) & 177 (1.785M) & 113 (1.14M) & 153 (1.544M) & 132 (1.33M)  \\
\bottomrule
\end{tabular}}
\end{table}

==> Tables/tab_mipnerf.tex <==
\begin{table}[ht]
\centering
\caption{\textbf{Per-scene rendering quality evaluation for Mip-NeRF360~\cite{barron2022mipnerf360} dataset.}}
\label{tab:mipnerf}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
Scene & \multicolumn{3}{c}{bicycle} & \multicolumn{3}{c}{garden} & \multicolumn{3}{c}{stump} & \multicolumn{3}{c}{room} & \multicolumn{3}{c}{counter} & \multicolumn{3}{c}{kitchen} & \multicolumn{3}{c}{bonsai} \\
\midrule
Method & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS \\
\midrule

{3D-GS~\cite{kerbl3Dgaussians}} & \cellcolor{tabsecond}25.25 & \cellcolor{tabfirst}{0.771} & \cellcolor{tabfirst}{0.205} & \cellcolor{tabfirst}{27.41} & \cellcolor{tabfirst}{0.868} & \cellcolor{tabfirst}{0.103} & \cellcolor{tabsecond}26.55 & \cellcolor{tabthird}0.775 & \cellcolor{tabfirst}{0.210} & 30.63 & 0.914 & 0.220 & 28.70 & 0.905 & 0.204 & 30.32 & \cellcolor{tabthird}0.922 & 0.129 & 31.98 & 0.938 & 0.205 \\

{MNeRF360~\cite{barron2022mipnerf360}} & 24.37 & 0.685 & 0.301 & 26.98 & 0.813 & 0.170 & \cellcolor{tabthird}26.40 & 0.744 & \cellcolor{tabthird}0.261 & 31.63 & 0.913 & 0.211 & \cellcolor{tabsecond}29.55 & 0.894 & 0.204 & \cellcolor{tabfirst}{32.23} & 0.920 & \cellcolor{tabthird}0.127 & \cellcolor{tabsecond}33.46 & \cellcolor{tabthird}0.941 & \cellcolor{tabsecond}0.176 \\

{iNPG~\cite{muller2022instant}} & 22.19 & 0.491 & 0.487 & 24.60 & 0.649 & 0.312 & 23.63 & 0.574 & 0.450 & 29.27 & 0.855 & 0.301 & 26.44 & 0.798 & 0.342 & 28.55 & 0.818 & 0.254 & 30.34 & 0.890 & 0.227 \\

{Plenoxels~\cite{yu2022plenoxels}} & 21.91 & 0.496 & 0.506 & 23.49 & 0.606 & 0.386 & 20.66 & 0.523 & 0.503 & 27.59 & 0.841 & 0.419 & 23.62 & 0.759 & 0.441 & 23.42 & 0.648 & 0.447 & 24.67 & 0.814 & 0.398 \\

{Scaffold-GS} &
\cellcolor{tabthird}24.50 & 0.705 & 0.306 &
\cellcolor{tabthird}27.17 & \cellcolor{tabsecond}0.842 & \cellcolor{tabsecond}0.146 &
26.27 & \cellcolor{tabfirst}{0.784} & 0.284 &
\cellcolor{tabsecond}31.93 & \cellcolor{tabsecond}0.925 & \cellcolor{tabsecond}0.202 &
\cellcolor{tabthird}29.34 & \cellcolor{tabsecond}0.914 & \cellcolor{tabsecond}0.191 &
\cellcolor{tabthird}31.30 & \cellcolor{tabsecond}0.928 & \cellcolor{tabsecond}0.126 &
32.70 & \cellcolor{tabsecond}0.946 & \cellcolor{tabthird}0.185 \\
\midrule

{SAGS-Lite} 
% bicycle
& 24.41 & \cellcolor{tabthird}0.719 & \cellcolor{tabthird}0.287 & 
% garden
25.62 & 0.775 & 0.230 & 
% stump
25.17 & 0.706 & 0.317 & 
% room
\cellcolor{tabthird}31.67 & \cellcolor{tabthird}0.923 & \cellcolor{tabthird}0.203 & 
% counter
28.93 & \cellcolor{tabthird}0.910 &\cellcolor{tabthird}0.194 & 
% kitchen
30.70 & 0.921 & 0.137 & 
% bonsai
\cellcolor{tabthird}33.31 & 0.933 & 0.210  \\ 

{SAGS} 
% bicycle
& \cellcolor{tabfirst}{25.30} & \cellcolor{tabsecond}0.759 & \cellcolor{tabsecond}0.231 %0.241 
% garden
& \cellcolor{tabsecond}27.25 & \cellcolor{tabthird}0.837 & \cellcolor{tabthird}0.151 %0.161 
% stump
& \cellcolor{tabfirst}{26.87} & \cellcolor{tabsecond}0.776 & \cellcolor{tabsecond}0.230 %0.242 
% room
& \cellcolor{tabfirst}{32.27} & \cellcolor{tabfirst}{0.933} & \cellcolor{tabfirst}{0.183} %0.185 
% counter
& \cellcolor{tabfirst}{29.86} & \cellcolor{tabfirst}{0.922} & \cellcolor{tabfirst}{0.176}
% kitchen
& \cellcolor{tabsecond}31.96 & \cellcolor{tabfirst}{0.935} & \cellcolor{tabfirst}{0.115}
% bonsai
& \cellcolor{tabfirst}{34.04} & \cellcolor{tabfirst}{0.955} & \cellcolor{tabfirst}{0.167}\\
\bottomrule
\end{tabular}}
\end{table}

==> Tables/tab_sizes.tex <==
\begin{table}[]
\centering
\caption{\textbf{Storage size (MB) comparison between the proposed and the baseline methods}. The proposed method achieves high fidelity rendering quality while effectively reducing the storage requirements of the scene.  
% The normalized memory measures how many times the baseline's memory consumption is compared with ours.
}
\vspace{-6pt}
\label{tab:mem_mip}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|cc|ccccccc}
\toprule
\begin{tabular}{c|c} Method & Scenes \end{tabular}  & Truck & Train & Dr Johnson & Playroom & bicycle&garden& stump&room&counter&kitchen&bonsai\\
\midrule

3D-GS~\cite{kerbl3Dgaussians} & 578 & 240 & 715 & 515 & 1291 & 1268 & 1034 & 327 & 261 & 414 & 281 \\
Scaffold-GS~\cite{lu2023scaffold} & 107 & 66 & 69 & 63 & 248 & 271 & 493 & 133 & 194 & 173 & 258 \\
\midrule
SAGS & \cellcolor{tabsecond}89 & \cellcolor{tabsecond}61 & \cellcolor{tabsecond}63 &\cellcolor{tabsecond}53 & \cellcolor{tabsecond}195 & \cellcolor{tabsecond}128 & \cellcolor{tabsecond}199 & \cellcolor{tabsecond}104 & \cellcolor{tabsecond}95 & \cellcolor{tabsecond}99 & \cellcolor{tabsecond}134 \\
SAGS-Lite & \cellcolor{tabfirst}40 & \cellcolor{tabfirst}29 & \cellcolor{tabfirst}32 & \cellcolor{tabfirst}24 & \cellcolor{tabfirst}113 & \cellcolor{tabfirst}76 & \cellcolor{tabfirst}103 & \cellcolor{tabfirst}52 & \cellcolor{tabfirst}42 & \cellcolor{tabfirst}43 & \cellcolor{tabfirst}77 \\
\bottomrule


\bottomrule
\end{tabular}

}
\end{table}
